Refinement types for precisely named cache locations

Many programming language techniques for incremental computation employ programmer-specified names for cached information. At runtime, each name identifies a "cache location" for a dynamic data value or a sub-computation; in sum, these cache location choices guide change propagation and incremental (re)execution. We call a cache location name precise when it identifies at most one value or subcomputation; we call all other names imprecise, or ambiguous. At a minimum, cache location names must be precise to ensure that change propagation works correctly; yet, reasoning statically about names in incremental programs remains an open problem. As a first step, this paper defines and solves the precise name problem, where we verify that incremental programs with explicit names use them precisely. To do so, we give a refinement type and effect system, and prove it sound (every well-typed program uses names precisely). We also demonstrate that this type system is expressive by verifying example programs that compute over efficient representations of incremental sequences and sets. Beyond verifying these programs, our type system also describes their dynamic naming strategies, e.g., for library documentation purposes.

==> Makefile <==
submit :
	./pull-abstract
	pdflatex typed-adapton
	bibtex typed-adapton
	pdflatex typed-adapton
	pdflatex typed-adapton
	mv typed-adapton.pdf supp.pdf
	pdflatex '\def\MainOnly{1} \input{typed-adapton.tex}'
	mv typed-adapton.pdf main.pdf



==> OLD-fig-nametermsorting.tex <==
\begin{figure}[t]
  \centering

  \judgbox{\Gamma |- M : \sort}
          {Under $\Gamma$,
            name term $M$ has sort $\sort$
          }
  \begin{mathpar}
    \Infer{M-const}
        {\Gamma |- n \wfname}
        {\Gamma |- n : \namesort}
    ~~~
    \Infer{M-abs}
        {\Gamma, a : \sort_1 |- M : \sort_2}
        {\Gamma |- (\lam{a} M) : (\sort_1 @> \sort_2)}
    ~~~
    \Infer{M-var}
        {(a : \sort) \in \Gamma}
        {\Gamma |- a : \sort}
    \and
    \Infer{M-app}
        {
          %\arrayenvbl{
          \Gamma |- M_1 : (\sort' @> \sort)
          \\
          \Gamma |- M_2 : \sort'
          %}
        }
        {\Gamma |- (M_1\;M_2) : \sort}
    \and
    \Infer{M-unit}
        {}
        {\Gamma |- \unitexp : \unitsort}
    \and
    \Infer{M-pair}
        {
          \Gamma |- M_1 : \sort_1
          \\
          \Gamma |- M_2 : \sort_2
        }
        {\Gamma |- \Pair{M_1}{M_2} : (\sort_1 * \sort_2)}
    \and
    \Infer{M-append}
        {
          \Gamma |- M : \namesort
        }
        {%\arrayenvbl{
           \Gamma |- M.1 : \namesort
           \\
           \Gamma |- M.2 : \namesort
         %}
         }
  \end{mathpar}

  \judgbox{\Gamma |- i : \sort}
          {Under $\Gamma$,
            index $i$ has sort $\sort$
          }
  \begin{mathpar}
    \Infer{sort-var}
        {
          (a : \sort) \in \Gamma
        }
        {
          \Gamma |- a : \sort
        }
    ~~~~~
    \Infer{sort-singleton}
        {
         %  \Gamma |- n \wfname
          \Gamma |- n : \namesort
        }
        {
          \Gamma |- \{n\} : \namesetsort
        }
    ~~~~~
    \Infer{sort-sep-union}
        {
          \Gamma |- X : \namesetsort
          \\
          \Gamma |- Y : \namesetsort
        }
        {
          \Gamma |- (X \disj Y) : \namesetsort
        }
    \and
    \Infer{sort-unit}
        {}
        {
          \Gamma |- \unitindex : \unitsort
        }
    \and
    \Infer{sort-pair}
        {
          \Gamma |- i_1 : \sort_1
          \\
          \Gamma |- i_2 : \sort_2
        }
        {
          \Gamma |- \Pair{i_1}{i_2} : (\sort_1 * \sort_2)
        }
    \\
    \Infer{sort-apply}
        {
          \Gamma |- M : \sort_1 @> \sort_2
          \\
          \Gamma |- i : \sort_1
        }
        {
          \Gamma |- M[[i]] : \sort_2
        }
    \and
    \Infer{sort-apply-pointwise}
        {
          \Gamma |- M : \namesort @> \namesort
          \\
          \Gamma |- i : \namesetsort
        }
        {
          \Gamma |- M[[i]] : \namesetsort
        }
  \vspace*{-1.5ex}
  \end{mathpar}

  \caption{Name term sorting and index sorting}
  \label{fig:sorting-rules}
\end{figure}


==> OLD-fig-syntax-compact.tex <==
\begin{figure}[htbp]
  \centering
 
\begin{grammar}
  Kinds
  & $K$
      &$\bnfas$&
      $\type$
      \\ &&& $\bnfaltbrk \type => K$ & type argument (binder space)
      \\ &&& $\bnfaltbrk \sort => K$ & index argument (binder space)
  \\[1ex]
  Name terms
 &$M$
      &$\bnfas$&
      $n$ & name
 \\ &&& $\bnfaltbrk \unitexp$ & unit
 \\ &&& $\bnfaltbrk \lam{a} M$ & abstraction
 \\ &&& $\bnfaltbrk a$ & variable
 \\ &&& $\bnfaltbrk \idxapp{M}{M}$ & application
 \\ &&& $\bnfaltbrk M.1$ & append 1 to name
 \\ &&& $\bnfaltbrk M.2$ & append 2 to name
 \\ &&& $\bnfaltbrk \Pair{M_1}{M_2}$ & tuple
%   \\ &&& $\bnfaltbrk t_1 \union t_2$ & union
  \\[1ex]
  Index sorts
  & $\sort$
      &$\bnfas$&
      $\namesort$  & name
   \\ &&& $\bnfaltbrk \namesetsort$   & name set sort
   \\ &&& $\bnfaltbrk \unitsort$   & unit index sort
   \\ &&& $\bnfaltbrk \sort * \sort$  & product index sort
   \\ &&& $\bnfaltbrk \sort @> \sort$ & index-level function
  \\[1ex]
%   Symbols
%   & $s$
%   \\[1ex]
  Names
  & $n, m, p, q$
     &$\bnfas$&
%      $s$  & symbol
%   \\ &&& $\bnfaltbrk$
           $\rootname$  & root name
   \\ &&& $\bnfaltbrk n.1 \bnfalt n.2$   & append bit (disjunctive names)
   \\ &&& $\bnfaltbrk \Pair{n_1}{n_2}$   & pairing (conjunctive names)
%  \\[1ex]  Name set variables  & $\namevar$    Use `a'
%   \\
%   Name sets
%   & \hspace{-4ex}$X, Y, Z, R, W$
%       &$\bnfas$&
%       $a$ &
%  \\ &&&
  \\[1ex]
  Index variables
  & $a$
  \\
  Index expressions
  & $i, X, Y, Z, R, W$
      &$\bnfas$&
      $a$
 \\ &&& $\bnfaltbrk \{n\}$ & singleton set
 \\ &&& $\bnfaltbrk X \disj Y$ & separating union
 \\ &&& $\bnfaltbrk \unitindex
      \bnfalt \Pair{i}{i}
      \bnfalt M[[i]]
      $
%   \\[1ex]
%   Propositions
%   & $P$
%       &$\bnfas$&
%       $
%       \trueprop
%       \bnfaltBRK P \andprop P
%       \bnfaltBRK X \disj Y
%       \bnfaltBRK X \subseteq Y
%       $
\end{grammar}

  \caption{Syntax for indices}
  \label{fig:syntax-indices}
\end{figure}



\begin{figure}[htbp]
  \centering
 
\begin{grammar}
  Effects
  & $\e$
      &$\bnfas$&
               $<<W; R>>$
  \\[1ex]
  Type constructors
  & $d$
  \\
  Type variables
  & $\alpha$
  \\
  Value types
  & $A, B$
      &$\bnfas$&
            $\alpha$ & type variable
      \\ &&& $\bnfaltbrk d$         & type constructor
      \\ &&& $\bnfaltbrk A + B$ & sum
      \\ &&& $\bnfaltbrk  A ** B$ & product
      \\ &&& $\bnfaltbrk  \Unit$
      \\ &&& $\bnfaltbrk \Ref{i}{A}$  & named reference cell
      \\ &&& $\bnfaltbrk \Thk{i}{E}$  & named thunk (with effects) % thunk
%      \\ &&& $\bnfaltbrk \Unthk{i}{E}$  & named ``unthunk'' (no effects) % unthunk
      \\ &&& $\bnfaltbrk  A[[i]]$  & application of type to index
      \\ &&& $\bnfaltbrk  A\;B$  & application of type constructor to type
      \\ &&& $\bnfaltbrk  \Name{i}$  & name type (name contained in name set $i$)
      \\ &&& $\bnfaltbrk  (\namesort @> \namesort)[[M]]$  & name function type (singleton)
  \\[1ex]
  Computation types
  & $C, D$
      &$\bnfas$&
      $\F A$  & li$\xF$t
 \\ &&& $\bnfaltbrk A -> E$    & function
  \\[1ex]
  \dots with effects
  & $E$
      &$\bnfas$&
      $C |> \e$  & effects
 \\ &&& $\bnfaltbrk \All{\alpha : K} E  $   & type polymorphism
% % \\ &&& $\bnfaltbrk \Univ{a : \sort} E  $   & index polymorphism
 \\ &&& $\bnfaltbrk \All{a : \sort} E  $   & index polymorphism
% % \\ &&& $\bnfaltbrk \Namearr{a}{\sort} E$   & name function polymorphism
%  \\ &&& $\bnfaltbrk P --> E  $   & guarded type
 \\[1ex]
  Typing contexts
  & $\Gamma$
    &$\bnfas$&
    $\cdot$
  \\ &&& $\bnfaltbrk \Gamma, p : A$ & ref pointer
  \\ &&& $\bnfaltbrk \Gamma, p : E$ & thunk pointer
  \\ &&& $\bnfaltbrk \Gamma, x : A$ & value variable
%  \\ &&& $\bnfaltbrk \Gamma, P$ & truth of proposition
\end{grammar}
\vspace*{-1.5ex}

  \caption{Syntax for types}
  \label{fig:syntax-types}
\end{figure}


% Local Variables:
% mode: latex
% TeX-master: "typed-adapton"
% End:


==> OLD-fig-syntax.tex <==
\begin{figure}[htbp]
  \centering
 
\begin{grammar}
  Kinds
  & $K$
      &$\bnfas$&
      $\type$
      \\ &&& $\bnfaltbrk \type => K$ & type argument (binder space)
      \\ &&& $\bnfaltbrk \sort => K$ & index argument (binder space)
  \\[1ex]
  Name terms
 &$M$
      &$\bnfas$&
      $n$ & name
 \\ &&& $\bnfaltbrk \unitexp$ & unit
 \\ &&& $\bnfaltbrk \lam{a} M$ & abstraction
 \\ &&& $\bnfaltbrk a$ & variable
 \\ &&& $\bnfaltbrk \idxapp{M}{M}$ & application
 \\ &&& $\bnfaltbrk M.1$ & append 1 to name
 \\ &&& $\bnfaltbrk M.2$ & append 2 to name
 \\ &&& $\bnfaltbrk \Pair{M_1}{M_2}$ & tuple
%   \\ &&& $\bnfaltbrk t_1 \union t_2$ & union
  \\[1ex]
  Index sorts
  & $\sort$
      &$\bnfas$&
      $\namesort$  & name
   \\ &&& $\bnfaltbrk \namesetsort$   & name set sort
   \\ &&& $\bnfaltbrk \unitsort$   & unit index sort
   \\ &&& $\bnfaltbrk \sort * \sort$  & product index sort
   \\ &&& $\bnfaltbrk \sort @> \sort$ & index-level function
  \\[1ex]
  Symbols
  & $s$
  \\[1ex]
  Names
  & $n, m, p, q$
     &$\bnfas$&
      $s$  & symbol
   \\ &&& $\bnfaltbrk \rootname$  & root name
   \\ &&& $\bnfaltbrk n.1 \bnfalt n.2$   & append bit (disjunctive names)
   \\ &&& $\bnfaltbrk \Pair{n_1}{n_2}$   & pairing (conjunctive names)
%  \\[1ex]  Name set variables  & $\namevar$    Use `a'
%   \\
%   Name sets
%   & \hspace{-4ex}$X, Y, Z, R, W$
%       &$\bnfas$&
%       $a$ &
%  \\ &&&
  \\[1ex]
  Index variables
  & $a$
  \\
  Index expressions
  & $i, X, Y, Z, R, W$
      &$\bnfas$&
      $a$
 \\ &&& $\bnfaltbrk \{n\}$ & singleton set
 \\ &&& $\bnfaltbrk X \disj Y$ & separating union
 \\ &&& $\bnfaltbrk \unitindex
      \bnfalt \Pair{i}{i}
      \bnfalt M[[i]]
      $
%   \\[1ex]
%   Propositions
%   & $P$
%       &$\bnfas$&
%       $
%       \trueprop
%       \bnfaltBRK P \andprop P
%       \bnfaltBRK X \disj Y
%       \bnfaltBRK X \subseteq Y
%       $
\end{grammar}

  \caption{Syntax for indices}
  \label{fig:syntax-indices}
\end{figure}



\begin{figure}[htbp]
  \centering
 
\begin{grammar}
  Effects
  & $\e$
      &$\bnfas$&
               $<<W; R>>$
  \\[1ex]
  Type constructors
  & $d$
  \\
  Type variables
  & $\alpha$
  \\
  Value types
  & $A, B$
      &$\bnfas$&
            $\alpha$ & type variable
      \\ &&& $\bnfaltbrk d$         & type constructor
      \\ &&& $\bnfaltbrk A + B$ & sum
      \\ &&& $\bnfaltbrk  A ** B$ & product
      \\ &&& $\bnfaltbrk  \Unit$
      \\ &&& $\bnfaltbrk \Ref{i}{A}$  & named reference cell
      \\ &&& $\bnfaltbrk \Thk{i}{E}$  & named thunk (with effects) % thunk
%      \\ &&& $\bnfaltbrk \Unthk{i}{E}$  & named ``unthunk'' (no effects) % unthunk
      \\ &&& $\bnfaltbrk  A[[i]]$  & application of type to index
      \\ &&& $\bnfaltbrk  A\;B$  & application of type constructor to type
      \\ &&& $\bnfaltbrk  \Name{i}$  & name type (name contained in name set $i$)
      \\ &&& $\bnfaltbrk  (\namesort @> \namesort)[[M]]$  & name function type (singleton)
  \\[1ex]
  Computation types
  & $C, D$
      &$\bnfas$&
      $\F A$  & li$\xF$t
 \\ &&& $\bnfaltbrk A -> E$    & function
  \\[1ex]
  \dots with effects
  & $E$
      &$\bnfas$&
      $C |> \e$  & effects
 \\ &&& $\bnfaltbrk \All{\alpha : K} E  $   & type polymorphism
% % \\ &&& $\bnfaltbrk \Univ{a : \sort} E  $   & index polymorphism
 \\ &&& $\bnfaltbrk \All{a : \sort} E  $   & index polymorphism
% % \\ &&& $\bnfaltbrk \Namearr{a}{\sort} E$   & name function polymorphism
%  \\ &&& $\bnfaltbrk P --> E  $   & guarded type
 \\[1ex]
  Typing contexts
  & $\Gamma$
    &$\bnfas$&
    $\cdot$
  \\ &&& $\bnfaltbrk \Gamma, p : A$ & ref pointer
  \\ &&& $\bnfaltbrk \Gamma, p : E$ & thunk pointer
  \\ &&& $\bnfaltbrk \Gamma, x : A$ & value variable
%  \\ &&& $\bnfaltbrk \Gamma, P$ & truth of proposition
\end{grammar}
\vspace*{-1.5ex}

  \caption{Syntax for types}
  \label{fig:syntax-types}
\end{figure}


% Local Variables:
% mode: latex
% TeX-master: "typed-adapton"
% End:


==> discussion.tex <==
\section{Discussion}
\label{sec:discussion}

We use our core calculus type system from \Secref{sec:typesystem} as
the basis for a \emph{family} of core calculi for reasoning about
programs use caches with explicit names.

In particular, we discuss an extension for typing a mixture of
incremental and functional reactive programming.

\subsection{Functional reactive programming with explicit names.}

Functional reactive programming (FRP) models provide abstractions
for describing time-varying behavior, often using high-level
abstractions for streams and/or events.
%
Behind the scenes, a \emph{reactive loop} executes as the main thread
of control, re-executing code from the FRP program as time advances.
%
Based on \Secref{sec:typesystem}, we sketch a core calculus where these
reactive loops' bodies may be incorporated into a an incremental
program with change propagation.

\paragraph{Proposed static semantics.}
%
To statically approximate the effects of reactive loops, we propose
augmenting our notion of effects (tracking reads and writes,
\emph{now}) to additionally mark where \emph{delayed feedback effects}
occur, allowing programmers to combine such loops and general-purpose
incremental computing.
%
Now effects consist of triples~$<<R;W;F>>$ where name sets $R$, $W$
and $F$ give the read, write and nominal feedback sets, respectively.

To control nominal feedback, we propose the following two primitives:
%
\[
\Infer{delay}
{\Gamma |- v : \Nm[[X]] \\ \Gamma |- e : E }
{\Gamma |- \keyword{delay}(v,e) : \F \big( \Thk{X}{E} \big) |> <<\emptyset; \emptyset; X>> }
~~
\Infer{loop}
{\arrayenvbl{ \Gamma |- e_1 : A |> <<R; W; F>> \\ \Gamma |- e_2 : \textsf{Loop}~A |> <<R{\disj}F; W; F>>} }
{\Gamma |- \keyword{loop}(e_1,e_2) : \F A |> <<R{\disj}W{\disj}F; W{\disj}F; \emptyset>>}
\]
%
The statics of the delay rule says that we can name a \emph{delayed}
thunk; the dynamic semantics of this primitive, discussed more below,
is to write this name (drawn from~$X$) with expression~$e$ \emph{just before the next
  loop iteration}.
%
(For simplicity here, we omit the write scope monad that is present in
the \Secref{sec:typesystem} rules; this can be easily added).
%
In the conclusion of the rule, we treat the loop's ``feedback writes''
like ordinary writes.
%
Within the loop, \code{let}-sequencing delayed writes works
analogously to ordinary writes: one cannot delay the same name twice.
Further, to restrict store updates to the loop iteration boundaries,
we do not permit the program to write and to also delay the same name.

To define loops, the programmer provides two expressions:
expression~$e_1$ creates the initial feedback state, performing
reads~$R$, writes~$W$ and delayed writes~$F$.  Expression~$e_2$ may
assume that $F$ has been written, and may read from it; by contrast,
the rule ``rewinds'' the write set~$W$, by \emph{not} assuming that it
has been written for $e_2$, which may re-perform these writes~$W$
(incrementally-updating prior allocations, like the \emph{editor}
would), and in the process, it may update (``re-delay'') thunks in~$F$
for the next loop iteration.

That sub-expression~$e_2$ has type $\textsf{Loop}~A |> \e$, which is a
computation that produces the following (recursive) sum type:
%
\[
\big(
  \textsf{Loop}~A |> \e
\big)
= 
\big(
  \F (A + \Thk{X}{(\textsf{Loop}_X~A) |> \e}) |> \e
\big)
\]
%
Statically, the expression $e_2$ will either produce a value of
type~$A$, or a thunk that produces more thunks (and perhaps possibly a
value) in the future.

\paragraph{Proposed dynamic semantics.}
The dynamic semantics of loops consist of re-running expression~$e_2$
until it produces its value (if ever) and in so doing, the write and
delay effects of expression~$e_2$ will typically \emph{overwrite} the
previous reads of $e_2$, creating an incrementalized feedback loop,
whose execution is guided by change propagation.

As mentioned above, the dynamic semantics treats delayed writes
specially, by delaying them until the \textsf{Loop} fully completes an
iteration.
%
This proposal corresponds closely with prior work on synchronous,
discrete-time FRP---especially~\citet{Krishnaswami13}.
%
A key difference is that in our programming model, we mix incremental
and reactive computations, and in both cases, names are explicitly
provided by the programmer.


==> fig-expr.tex <==
\begin{figure}[htbp]
  \centering
 
\begin{grammar}
  Values
  & $v$
      &$\bnfas$&
      $x$
      \\ &&& $\bnfaltbrk \unitexp$ & 
      \\ &&& $\bnfaltbrk \Pair{v_1}{v_2}$ & introduce product
      \\ &&& $\bnfaltbrk \inj{i}{v}$ & introduce sum
      \\ &&& $\bnfaltbrk \name{M}$ & the name $n$, as a value
      \\ &&& $\bnfaltbrk \namefn{M}$ & the name term $M$
      \\ &&& $\bnfaltbrk \refv{M}$ & ref cell at location $n$
      \\ &&& $\bnfaltbrk \thunk{M}$ & thunk at location $n$
%      \\ &&& $\bnfaltbrk \unthunk{n}$ &
  \\[1ex]
  Terminal expressions
  & $t$
      &$\bnfas$&
              $\Ret{v}$ & return the value $v$
      \\ &&& $\bnfaltbrk \lam{x} e$ & ordinary $\lambda$
  \\[1ex]
  Expressions
  & $e$
      &$\bnfas$&
           $t$ & terminal expression (above)
      \\ &&& $\bnfaltbrk \Split{v}{x_1}{x_2}{e}$ & eliminate product
      \\ &&& $\bnfaltbrk \Case{v}{x_1}{e_1}{x_2}{e_2}$ & eliminate sum
%      \\ &&& $\bnfaltbrk \Ret{v}$ & return the value $v$
%      \\ &&& $\bnfaltbrk \lam{x} e$ & ordinary $\lambda$
      \\ &&& $\bnfaltbrk \Let{e_1}{x}{e_2}$ &
      \\ &&& $\bnfaltbrk e\;v$ & ordinary function application
      \\ &&& $\bnfaltbrk \Refe{v} v$ & allocate a ref cell
      \\ &&& $\bnfaltbrk \Thunk{v} e$ & create a thunk
%      \\ &&& $\bnfaltbrk \Unthunk{v}$ &
      \\ &&& $\bnfaltbrk \Force{v}$ & force a thunk
      \\ &&& $\bnfaltbrk \Get{v}$ & get the contents of a ref cell
%      \\ &&& $\bnfaltbrk \Ns{v}{e}$ &
      \\ &&& $\bnfaltbrk \Scope{M}{e}$ & enter a namespace
      \\ &&& $\bnfaltbrk v_1\;v_2$ & name function $v_1$ applied to name $v_2$
%      \\ &&& $\bnfaltbrk \namearrintro{a}{e}$ & intro.\ form for $\Namearrsym$
%      \\ &&& $\bnfaltbrk \namearrelim{e}{t}$ & elim.\ form for $\Namearrsym$
\end{grammar}

  \caption{Syntax of expressions}
  \label{fig:expr}
\end{figure}


% Local Variables:
% mode: latex
% TeX-master: "types"
% End:


==> fig-inc-dynamics.tex <==
\begin{figure}[thbp]

\begin{grammar}
Graphs 
& $G$,$H$
    & $\bnfas$ & $\cdots$
\\ &&& $\bnfaltbrk$ $G, p {:} ( e , t )\,{@}\,M$ & $p$ points to thunk $e$ in namespace $M$ with cached result $t$
\\ &&& $\bnfaltbrk$ $G, (p, a, b, q)$ & $p$ depends on $q$ due to action $a$ with status $b$

\\[1ex]

Edge actions
& $a$ 
  & $\bnfas$ & &
   \text{For edge $(p, a, b, q)$, the computation at $p$\dots}
\\ &&&              $\textsf{alloc} \, v$ & $\dots$ created reference $v$ at $q$
\\ &&& $\bnfaltbrk$ $\textsf{alloc} \, e$ & $\dots$ created thunk $e$ at $q$
\\ &&& $\bnfaltbrk$ $\textsf{obs} \, v  $ & $\dots$ read $q$'s value, which was $v$
\\ &&& $\bnfaltbrk$ $\textsf{obs} \, e  $ & $\dots$ forced thunk $q$, which normalized as $e$

\\[1ex]

Edge statuses
& $b$ 
  & \bnfas 
     & \textsf{clean} 
     & value or computation at sink is out of date
\\ &&& $\bnfaltbrk$ \textsf{dirty} 
     & value or computation at sink is up to date
\end{grammar}

\caption{Graphs with structure for incremental computation: cached results and dependency edges}
\label{fig:graph-incremental}
\end{figure}

\begin{figure}[htbp]
  \centering

  %% \judgbox
  %%     {e \terminal}
  %%     {Expression $e$ is terminal}
  %% \vspace{-2ex}
  %% \begin{mathpar}
  %%   \Infer{}
  %%       {}
  %%       {\Ret{v} \terminal}
  %%   \and
  %%   \Infer{}
  %%       {}
  %%       {(\lam{x} e) \terminal}
  %%   \and
  %%   \Infer{}
  %%       {}
  %%       {(\namearrintro{a}{e}) \terminal}
  %% \end{mathpar}
  
  \judgbox{\PreSt{G_1}{M}{m} e !! G_2 ; e'}{
    Under graph $G_1$, namespace $M$ and current node $m$, 
    $e$ produces $G_2$ and $e'$.}
\begin{mathpar}\end{mathpar}
\\[-7mm]
\colorbox{light-gray}{
  \begin{mathpar}
    \small
    \Infer{thunk-clean}
      {
        (M\,p) \nteval q
        \\
        \textsf{exp}(G, q) = e
        \\
        \textsf{ns}(G, q) = M
      }
      {
        \PreSt{G} {M}{m} \Thunk{\name{p}} e !! 
        G, (m,\textsf{alloc}\,e,\textsf{clean},q); \Ret{\thunk{q}}
      }
    \and
    \Infer{thunk-dirty}
      {
        (M\,p) \nteval q
        \\ 
        G_1\{q{\mapsto}e\,{@}\,M\} = G_2
        \\
        \textsf{dirty-paths-in}(G_2, q) = G_3 
      }
      {
        \PreSt{G_1} {M}{m} \Thunk{\name{p}} e !! 
        G_3, (m,\textsf{alloc}\,e,\textsf{clean},q); \Ret{\thunk{q}}
      }
    \and
    \Infer{ref-clean}
        {
          (M\,p) \nteval q
          \\ 
          G(q) = v
        }
        {
          \PreSt{G} {M}{m} \Refe{\name{p}}{v} !! 
          G, (m,\textsf{alloc}\,v,\textsf{clean},q); \Ret{\refv{q}}
        }
    \and
    \Infer{ref-dirty}
        {
          (M\,p) \nteval q
          \\ 
          G_1\{p{\mapsto}v\} = G_2 
          \\ 
          \textsf{dirty-paths-in}(G_2, p) = G_3 
        }
        {
          \PreSt{G_1} {M}{m} \Refe{\name{p}}{v} !! 
          G_3, (m,\textsf{alloc}\,v,\textsf{clean},q); \Ret{\refv{q}}
        }
    \and
    \Infer{force-clean}
        {
          G_1 |- p *> G_2 ; t
%          \\
%          G_2(p) = (e, t)\,{@}\,m_0
        }
        {
          \PreSt{G_1} {M}{m} \Force{\thunk{p}} !! 
          G_2, (m,\textsf{obs}\,t,\textsf{clean},p); t
        }
    \and
    \Infer{get-clean}
      { G(q) = v }
      { \PreSt{G} {M}{m} \Get{\refv{q}} !! 
        G, (m,\textsf{obs}\,v,\textsf{clean},q); \Ret{v} }
  \end{mathpar}
  }
  \caption{Incremental evaluation rules: Ref and thunk reuse guided by dirtying and cleaning the DCG.}
  \label{fig:dynamics-incremental}
  \label{fig:inc-dynamics}

\vspace*{5mm}

 \judgbox{G_1 |- p *> G_2 ; t}{
    Under graph $G_1$, cleaning the DCG rooted at node $p$ produces $G_2$ and $t$.}

\begin{mathpar}
    \Infer{clean-done}
        {
          \textsf{all-clean-out}(G, p)
          \\\\
          G(p) = (e, t)\,{@}\,M
        }
        {
          G |- p *> G; t
        }
    \and
    \Infer{clean-edge}
      {
        \arrayenvbl{
          \textsf{all-clean-out}((G_1, G_2), q_2)
          \\
          \textsf{consistent-action}((G_1, G_2), a, q_2)
          \\
          G_1, (q_1, a, \textsf{clean}, q_2), G_2 |- p *> G_3; t
        }
      }
      {
        G_1, (q_1, a, \textsf{dirty}, q_2), G_2 |- p *> G_3; t
      }
    \and
    \Infer{clean-node}
      {
        \arrayenvbl{
          \big(\textsf{exp}(G_1, q) = e\big)
          \wedge
          \big(\textsf{ns}(G_1, q) = M\big)
          \\
          \textsf{del-edges-out}(G_1\{q \mapsto e\,{@}\,M\}, q) = G_1'
          \\
          \D :: \PreSt{G_1'}{M}{q} e !! G_2; t
          \\
          \Cc :: G_2\{q \mapsto (e, t)\} |- p *> G_3, t'
          \\
          \DHasEffects{\D}{R_\D}{W_\D} \Rightarrow \big(
            (\DHasEffects{\Cc}{R_\Cc}{W_\Cc})
            \wedge
            (W_\D \disjoint W_\Cc)
            \wedge
            (R_\D \disjoint W_\Cc)
          \big)
        }
      }
      {
        G_1 |- p *> G_3; t'
      }
\end{mathpar}

  \caption{Incremental cleaning rules: Cleaning graph nodes and edges.}
  \label{fig:dynamics-clean}

\end{figure}


==> fig-listmap.tex <==

\subsection{Example Series: List Map}

\paragraph{Functional Programming with Names}

The type below defines incremental lists of integers.  
%
Specifically, the type $\List{X}{Y}{\Int}$ classifies lists that
consist of integers, names from set~$X$, and (incrementally changing)
references whose pointer names are drawn from set~$Y$.

\[
\begin{array}{rcrrll}
\keyword{Nil}  &:& \All{X,Y} &&&\List{X}{Y}{\Int}
\\
\keyword{Cons} &:& \All{X,Y} &\Int -> &\List{X}{Y}{\Int} -> &\List{N}{M}{\Int}
\\
\keyword{Name} &:& \All{X_1,X_2,Y} &\Name{X_1} -> &\List{X_2}{Y}{\Int} -> &\List{X_1\disj X_2}{Y}{\Int}
\\
\keyword{Ref}  &:& \All{X,Y_1,Y_2} &\multicolumn{2}{r}{\Ref{Y_1}{} (\List{X}{Y_2}{\Int})}\!\!$\rightarrow$ & \List{X}{Y_1\disj Y_2}{\Int}
\end{array}
\]

The type $\List{X}{Y}{\Int}$ has two conventional constructors,
\keyword{Nil} and \keyword{Cons}, as well as two additional
constructors, \keyword{Name} and \keyword{Ref}, for injecting
(disjoint) names and (incrementally changing) sub-lists into the list,
respectively.

\paragraph{TO DO}: Illustrate an example list here.

A computation that consumes a list of type $\List{X}{Y}{\Int}$ may use
the names in set~$X$ to name the structure of its output and
recursion.  In the process of consuming this list, a computation
observes references in the list, whose pointers are named by names in
set $Y$.  Once observed, these pointers may not be overwritten without
(potentially) affecting the results of computations that depend on
them.

Below, we consider a computation for mapping a list, which observes a
list and allocates another holding the mapped output elements.

\paragraph{TO DO}: Continue refactoring examples, below.
Before showing code that pairs names, show code that does not, show a
misuse, and then motivate the pairing code.

\paragraph{Mapping an incremental list of integers}

Consider the higher-order function \texttt{listmap} that, given a
function over integers, maps an input list of integers to an output
list in a pointwise fashion.
%
The \texttt{Nil} and \texttt{Cons} cases below are conventional;
%
In the \texttt{Name} case, the programmer injects the name~\texttt{n}
into the output list, but also uses it to name a thunk for a (lazy)
recursive call on the tail.
%
In particular, the name pair \texttt{(n0, n)} combines the input
list's name~\texttt{n} with a distinguished name~\texttt{n0}, provided
by the calling context.

\[
\begin{array}{l}
\All{N_0,N,M:\namesort}
\\
\Name{N_0}
\\
-> (\Int -> \Int)
\\
-> \List{N}{M}{\Int}
\\
-> \List{N}{\Pair{N_0}{N}}{\Int}
\end{array}
\]
\begin{verbatim}
listmap = lambda n0. lambda f. 
   fix listmap_rec. lambda l.
   match l with
    Nil       => Nil,
    Cons(h,t) => Cons(f h, listmap_rec t)
    Name(n,t) => Name(n, Art (thunk (n0, n) [ listmap_rec t) ])
    Art(a)    => listmap_rec (force a)
\end{verbatim}

\marginnote{Q: When to introduce read and write effects? Here?}

The name-pairing of \texttt{(n0, n)} in the \texttt{Name} case is
important; if the programmer had instead used only name \texttt{n},
then two distinct uses of map will name their thunks ambiguously,
using the same names of the same input list \texttt{inp}.
%
Because it is parametric in the function \texttt{f} and the
distinguished name \texttt{n0}, a calling context may use
\texttt{listmap} to instantiate different integer mappings, as
follows:

\begin{verbatim}
let x = listmap n1 abs inp 
let y = listmap n2 sq  inp
\end{verbatim}

Assuming that $n_1\disj n_2$, we have that the thunks in the outputs
\texttt{x} and \texttt{y} are distinct from each other.
%
Otherwise, if we had that $n_1 = n_2$, the map outputs would overwrite
each other's thunks; the order of this overwriting depends on how
\texttt{x} and \texttt{y} are (lazily) forced by the surrounding
evaluation context.
%
The type system proposed by this paper rules out overwriting that
leads to unsound results (that is, results that are inconsistent with
from-scratch execution).

Intuitively, the programmer avoids such behavior by distinguishing the
outputs of the two instantiations; above, she uses the distinguished
names \texttt{n1} and \texttt{n2}.
\marginnote{Mention write effects?}

\paragraph{Name Function Parametricity}

When writing reusable library code, the programmer may want to avoid
choosing the specifics of how to name output structure. For instance,
when naming the lazy thunk in the \keyword{Name} case above, rather
than choose to pair the names~$n0$ and $n$, she may want to be more
generic, and defer even more decisions to the calling context.
%
To express this generality, she parameterizes \keyword{listmap} with a
name-transforming function \keyword{fnm}.
%
The articulations of the output list type are named by applying
\keyword{fnm} to the names of the input list.
%
In terms of program text, this generalization universally quantifies
over the name function~\texttt{fnm}, and it applies this function in
the \texttt{Name} case.
%
Compared to the version above that is parametric in a distinguished
name~\texttt{n0}, this version is more general; to recover the first
version, let the name function~\texttt{fnm} be one that pairs its
argument with the distinguished name~\texttt{n0}.


\[
\begin{array}{l}
\All{\texttt{fnm}: \namesort @> \namesort}
\\
\All{X,Y: \namesetsort}
\\
(\Int -> \Int)
\\
->
\List{X}{Y}{\Int}
\\
-> \List{X}{\texttt{fnm}~Y}{\Int}
\end{array}
\]
\begin{verbatim}
listmap f l = forall fnm. lambda f. 
   fix listmap_rec. lambda l.
   match l with
    Nil       => Nil,
    Cons(h,t) => Cons(f h, listmap_rec t)
    Name(n,t) => Name(n, Art (thunk (fnm n) [ listmap_rec t) ])
    Art(a)    => listmap_rec (force a)
\end{verbatim}

\paragraph{Map Function Parametricity}

Suppose we want a map function that works over any type of lists, not
just lists of integers.  To do so, we want the computation to be
generic in the structures of the input and output list, and their
naming relationships.
%
The programmer achieves this generality by abstracting over several
structure-specific choices: The input and output list's type
structure, call them $A$ and $B$, as well as the index structure of
these types, and their relationship.
%
In particular, we introduce another name function~\texttt{fab} to
abstract over the ways that names in type~$A$ are used to index the
names of type~$B$.
%
To classify the types $A$ and $B$, we use the kinds $k_A => \type$ and
$k_B => \type$, respectively; the index sorts $k_A$ and $k_B$ classify
the nominal indices of these types, and the index sort $k_A @> k_B$
classifies the name function~\texttt{fab}, which relates names of
type~$A$ to names of type~$B$.

\[
\begin{array}{l}
\Univ{k_A:\sort}\All{A:k_A => \type}
\\
\Univ{k_B:\sort}\All{B:k_B => \type} 
\\
\All{\texttt{fab}: k_A @> k_B}
\\
\All{\texttt{fnm}: \namesort @> \namesort}
\\
\All{N,M:\namesort}\All{X:k_A}
\\
% (\All{X':k_A} (X' \subseteq X) --> A\tbrack{X'} -> B\tbrack{\texttt{fab}\;X'})
~~~~(A\tbrack{X} -> B\tbrack{\texttt{fab}\;X})
\\
~~-> \List{N}{M}{A\tbrack{X}}
\\
~~-> \List{N}{\texttt{fnm}~N}{B\tbrack{\texttt{fab}\;X}}
\end{array}
\]


\paragraph{Eager and Lazy Structures}

We often want to express computations that consume both eager and lazy
data structures in a uniform fashion.
%
To do so, we introduce the concept of an ``articulation'', which is
either a lazy thunk that produces a value of type $A$ when forced, or
a write-once reference cell that holds a value of type $A$:
\[
\begin{array}{rclll}
\Art{N}{A} &=& \keyword{AThunk}&\keyword{of}~&\U\tbrack{N}(\F{A})
\\
           &|& \keyword{ARef}&\keyword{of}~&\Ref{N}{A}
\end{array}
\]
Like both thunks and reference cells, an articulation's type is
indexed by a name set.
\marginnote{To start, we can just use ref cells in lists.  But where should we push the discussion of articulations?}
\marginnote{
Question: How to justify erasing the Thunk's effects from the types of articulations?
}
\marginnote{
Can we prove that the written names are in the history?
(If we know that the effects of the art are consistent with history, and apart of it, we can erase them)
}

% Local Variables: 
% mode: latex
% TeX-master: types
% End: 


==> fig-namestep.tex <==



\THIS\FIGURE\IS\OBSOLETE



\begin{figure}[t]
  \centering

  \begin{grammar}
      Name term values
     &$\Mv$
          &$\bnfas$&
          $n
          \bnfalt \lam{a} M
          \bnfalt a
          \bnfalt \unitexp
          \bnfalt \Pair{\Mv}{\Mv}
          \bnfalt \Mv.1
          \bnfalt \Mv.2
          $
  \end{grammar}

  \judgbox{M \nteval \Mv}
          {Name term $M$ evaluates to name term value $\Mv$
          }
  \begin{mathpar}
    \Infer{teval-value}  % name, abstraction, [variable], unit
       {}
       {\Mv \nteval \Mv}
    \and
    \Infer{teval-app}
        {
          M_1 \nteval \lam{a} M
          \\
          M_2 \nteval \Mv_2
          \\
          [\Mv_2 / a]M \nteval \Mv
        }
        {(M_1\,M_2) \nteval \Mv}
    \and
    \Infer{teval-pair}
        {
          M_1 \nteval \Mv_1
          \\
          M_2 \nteval \Mv_2
        }
        {
          \Pair{M_1}{M_2} \nteval \Pair{\Mv_1}{\Mv_2}
        }
    \and    
    \Infer{teval-append}
        {
          M \nteval \Mv
        }
        {
          \arrayenvbl{
            M.1 \nteval \Mv.1
            \\
            M.2 \nteval \Mv.2
          }
        }     
  \vspace*{-2ex}
  \end{mathpar}

  \caption{Name term evaluation}
  \label{fig:namestep}
\end{figure}


% Local Variables:
% TeX-master: "types"
% End:


==> fig-syntax-types-compact.tex <==
\begin{figure}[t]
  \centering
 
\begin{grammar}
  Name terms
 &$M$
      &$\bnfas$&
      $n 
\bnfalt \unitexp
 \bnfalt \lam{a} M
 \bnfalt a
 \bnfalt \idxapp{M}{M}
 \bnfalt M.1
 \bnfalt M.2
 \bnfalt \Pair{M_1}{M_2}
$
  \\[0.6ex]
  Index sorts
  & $\sort$
      &$\bnfas$&
      $\namesort
   \bnfalt \namesetsort
   \bnfalt \unitsort
   \bnfalt \sort * \sort
   \bnfalt \sort @> \sort$
  \\[0.6ex]
%   Symbols
%   & $s$
%   \\[0.6ex]
  Names
  & $n, m, p, q$
     &$\bnfas$&
$ \rootname
   \bnfalt n.1 \bnfalt n.2
   \bnfalt \Pair{n_1}{n_2}$
  \\[0.6ex]
  Index variables
  & $a$
  \\
  Index exprs.
  & $i, X, Y, Z, R, W$
      &$\bnfas$&
      $a
 \bnfalt \{n\}
 \bnfalt X \disj Y
 \bnfalt \unitindex
      \bnfalt \Pair{i}{i}
      \bnfalt M[[i]]
      $
\end{grammar}
\vspace*{-1.0ex}

  \caption{Syntax of indices, including names}
  \label{fig:syntax-indices}
\end{figure}



\begin{figure}[htbp]
  \centering
 
\begin{grammar}
  Kinds
  & $K$
      &$\bnfas$&
      $\type
      \bnfalt \type => K
      \bnfalt \sort => K
      $
%   \\[0.6ex]
%   Propositions
%   & $P$
%       &$\bnfas$&
%       $
%       \trueprop
%       \bnfaltBRK P \andprop P
%       \bnfaltBRK X \disj Y
%       \bnfaltBRK X \subseteq Y
%       $
  \\[0.6ex]
  Effects
  & $\e$
      &$\bnfas$&
               $<<W; R>>$
  \\[0.6ex]
  Type constructors
  & $d$
  \\
  Type variables
  & $\alpha$
  \\
  Value types
  & $A, B$
      &$\bnfas$&
            $\alpha
      \bnfalt d
      \bnfalt A + B
      \bnfalt  A ** B
      \bnfalt  \Unit
      \bnfalt \Ref{i}{A}
      \bnfalt \Thk{i}{E}
%      \bnfalt \Unthk{i}{E}$  & named ``unthunk'' (no effects) % unthunk
      \bnfaltBRK  A[[i]]
      \bnfalt  A\;B
      \bnfalt  \Name{i}
      \bnfalt  (\namesort @> \namesort)[[M]]$
  \\[0.6ex]
  Computation types
  & $C, D$
      &$\bnfas$&
      $\F A
 \bnfalt A -> E$
  \\[0.6ex]
  \dots with effects
  & $E$
      &$\bnfas$&
      $C |> \e
 \bnfalt \All{\alpha : K} E
% % \bnfalt \Univ{a : \sort} E  $   & index polymorphism
 \bnfalt \All{a : \sort} E  $
% % \bnfalt \Namearr{a}{\sort} E$   & name function polymorphism
%  \bnfalt P --> E  $   & guarded type
 \\[0.6ex]
  Typing contexts
  & $\Gamma$
    &$\bnfas$&
    $\cdot
  \bnfalt \Gamma, p : A
  \bnfalt \Gamma, p : E
  \bnfalt \Gamma, x : A$
%  \bnfalt \Gamma, P$ & truth of proposition
\end{grammar}
\vspace*{-1.0ex}

  \caption{Syntax of kinds, effects and types}
  \label{fig:syntax-types}
\end{figure}


% Local Variables:
% mode: latex
% TeX-master: "typed-adapton"
% End:


==> meta-dynamics.tex <==
\section{Dynamics Metatheory: From-Scratch Consistency}
\Label{apx:metatheory}

\subsection{Overview}

Our main formal result in this paper, \emph{from-scratch consistency},
states that given an evaluation derivation
corresponding to an incremental computation, we can construct a derivation
corresponding to a non-incremental computation that returns the same result
and a corresponding graph.  That is, the incremental computation is consistent
with a computation in the simpler non-incremental system.

To properly state the consistency result, we need to define what it means for a graph to
be well-formed (\Sectionref{sec:graph-wf}),
%
relate the incremental computation's DCG
to the non-incremental computation's store (\Sectionref{sec:restriction}),
describe the sets of nodes read and written by an evaluation derivation
(\Sectionref{sec:rw-sets}),
and prove a store weakening lemma~(\Sectionref{sec:weakening}).
The consistency result itself is stated and proved in \Sectionref{sec:fsc}.



\subsection{Graph Well-Formedness}
\Label{sec:graph-wf}

\begin{figure*}
\small
%\ottdefnsGrwf
\begin{mathpar}
\Infer{Grwf-emp}
    { }
    {G |- \cdot \wf}
\and
\Infer{Grwf-ref}
    {G |- H \wf
    \\
    G(p) = v
    }
    {G |- H, p:v \wf}
\and
\Infer{Grwf-thunk}
    {G |- H \wf
    \\
    G(p) = e
    }
    {G |- H, p:e \wf}
\and
\Infer{Grwf-thunkCache}
    {
      G |- H \wf
      \\
      \arrayenvbl{
        G(p) = (e,e')
        \\
        \textsf{if}~\textsf{all-clean-out}(G,p)~\textsf{then}~\D \derives \PreSt{G}{p}{w} e !! G ; e'
        \\
        \textsf{if not}~\textsf{all-clean-out}(G, p)~\textsf{then}~\textsf{all-dirty-in}(G, p)
      }
    }
    {G |- H, p:(e,e') \wf}
\and
\Infer{Grwf-dirtyEdge}
    {
    G |- H \wf
    \\
    (p, a, \textsf{dirty}, q) \in G
    \\
    q \in \textsf{dom}(H)
    \\
    \textsf{if}~(p_0, a_0, b_0, p) \in G~\textsf{then}~b0 = \textsf{dirty}
    }
    {G |- H, (p, a, \textsf{dirty}, q) \wf}
\and
\Infer{Grwf-cleanEdge}
    {
    G |- H \wf
    \\
    (p, a, \textsf{clean}, q) \in G
    \\
    \textsf{consistent-action}(H, a, q)
    \\
    \textsf{all-clean-out}(G, q)
    }
    {G |- H, (p, a, \textsf{clean}, q) \wf}
\end{mathpar}
\vspace{-3ex}
\caption{Graph well-formedness rules}
\FLabel{fig:graph-wf}
\end{figure*}

The judgment $G |- H \wf$ is read ``$H$ is a well-formed subset of $G$''.
It implies that $H$ is a linearization of a subset of $G$: within $H$,
information sources appear to the left of information sinks,
dependency edges point to the left, and information flows to the right.
Consequently, $H$ is a dag.

For brevity, we write $G \wf$ for $G |- G \wf$, threading
the entire graph $G$ through the rules deriving $G |- H \wf$.
The well-formedness rules in \Figureref{fig:graph-wf} decompose the right-hand
graph, and work as follows:

\begin{itemize}
\item
  For values (Grwf-val) and thunks with no cached result (Grwf-thunk),
  the rules only check the correspondence between $G$ (the entire graph)
  and $H$ (the subgraph).

\item For thunks with a cached result, Grwf-thunkCache
  examines the outgoing edges.  If they are all clean, then it checks
  that evaluating $e$ \emph{again}
  would not change the graph at all: $\D \derives \PreSt{G}{p}{w} e !! G ; t$.
%  (It also checks that the derivation $\D$ is ``satisfactory''; see
%  \Sectionref{sec:satisfactory-derivations}.)
  If one or more edges are dirty, it checks that all incoming edges are dirty.

\item
  Grwf-dirtyEdge checks that
  all edges flowing into a dirty edge are dirty:
  given edges from $p$ to $q$ and from $q$ to $r$, where
  the edge from $q$ to $r$ is dirty (meaning that $q$ depends on $r$ and $r$ needs
  to be recomputed), the edge from $p$ to $q$ should
  also be dirty.  Otherwise, we would think we could reuse the result in $p$,
  even though $p$ (transitively) depends on $r$.

  Conversely, if an edge from $p$ to $q$ is clean (Grwf-cleanEdge),
  then all edges out from $q$ must
  be clean (otherwise we would contradict the ``transitive dirtiness'' just described).
  Moreover, the action $a$ stored in the edge from $p$ to $q$ must be consistent
  with the contents of $q$.
\end{itemize}


\subsection{From Graphs to Stores: the Restriction Function}
\Label{sec:restriction}

To relate the graph associated with an incremental evaluation to
the store associated with a non-incremental evaluation, we define
a function~$\restrict{G}{P}$ that restricts $G$ to a set of pointers
$P$, drops cached thunk results (*), and erases all edges (**):
%
\begin{defn}[Restriction]
\Label{def:restrict}
\[
  \begin{array}{cr@{~~}c@{~~}lll}
    &\restrict{\emptyset}{P} &=& \emptyset
    \\[1ex]
    &\restrict{G, p:v}{P} &=& \restrict{G}{P}, p:v & \text{if $p \in P$}
    \\
    &\restrict{G, p:v}{P} &=& \restrict{G}{P} & \text{if $p \notin P$}
    \\[1ex]
    &\restrict{G, p:e}{P} &=& \restrict{G}{P}, p:e & \text{if $p \in P$}
    \\
    &\restrict{G, p:e}{P} &=& \restrict{G}{P} & \text{if $p \notin P$}
    \\
    \text{(*)}&\restrict{G, p:(e,t)}{P} &=& \restrict{G}{P}, p:e & \text{if $p \in P$}
    \\
    &\restrict{G, p:(e,t)}{P} &=& \restrict{G}{P} & \text{if $p \notin P$}
    \\[1ex]
    \text{(**)}&\restrict{G, (p,a,b,q)}{P} &=& \restrict{G}{P}
  \end{array}
\]
\end{defn}



\paragraph{Agreement.}  We want to express a result
 (\Lemmaref{lem:respect-write}) that evaluation only affects pointers in the write set
$W$, leaving the contents of other pointers alone, so we define what it means
to leave pointers alone:

\begin{defn}[Agreement on a pointer]
  Graphs $G_1$ and $G_2$ \emph{agree on}
  $p$ iff either $G_1(p) = G_2(p)$,
  or $p:v \in G_1$ and $p:v \in G_2$.
\end{defn}

\begin{defn}[Agreement on a set of pointers]
  Graphs $G_1$ and $G_2$ \emph{agree on}
  a set $P$ of pointers iff $G_1$ and $G_2$
  agree on each $p \in P$.
\end{defn}

\begin{lem}[Respect for write-set]
\Label{lem:respect-write}
~\\
   If $\D \derives \PreSt{G}{p}{w} e !! G';t$ where $\D$ is incremental
%   \\
   and $\DHasEffects{\D}{R}{W}$
%   \\
%   and $\D \monotonic$
   \\
   then $G'$ agrees with $G$ on $\dom{G} - \dom{W}$.
\end{lem}
\begin{proof}
  By a straightforward induction on $\D$, referring to \Definitionref{def:rw}.

  In the Eval-forceClean case, use the fact that $G'$ differs
  from $G$ only in the addition of an edge, which does not affect agreement.
\end{proof}


\subsection{Satisfactory derivations}
\Label{sec:satisfactory-derivations}

In our main result~(\Theoremref{thm:fsc}), we will assume that all input
and output graphs appearing within a derivation are well-formed,
and that the read- and write-sets are defined:

\begin{defn}[Locally satisfactory]
\Label{def:local-sat}
~\\
     A derivation
     $\D \derives \PreSt{G_1}{p}{w} e !! G_2 ; t$
     is \emph{locally satisfactory}
     if and only if

     \begin{enumerate}[(1)]
     %
    \item  % (1)
           $G_1 \wf$ and $G_2 \wf$

     \item  % (2) ``functional''
           $\DHasEffects{\D}{R}{W}$ is defined

     \end{enumerate}
\end{defn}

\begin{defn}[Globally satisfactory]
\Label{def:global-sat}
~\\
    An evaluation derivation
    $\D \derives \PreSt{H_1}{p}{w} e !! H_2 ; t$
    is \emph{globally satisfactory}, written~$\D \satisfactory$,
    if and only if
    $\D$ is locally satisfactory
    and all its subderivations are locally satisfactory.
\end{defn}


\subsection{Weakening}
\Label{sec:weakening}

The main result needs to construct a non-incremental derivation
in a different order from the given incremental derivation.
In particular, the first evaluation $\D_1$ done in Eval-computeDep
will be done ``later'' in the non-incremental derivation.
Since it
is done later, the graph may have new material $G'$,
and we need a weakening lemma to move from a non-incremental
evaluation of $\D_1$ (obtained through the induction hypothesis)
to a non-incremental evaluation over the larger graph.

\begin{lem}[Weakening (non-incremental)]
\Label{lem:weakening-ni}
~\\
   If $\D \derives \PreSt{G_1}{p}{w} e !! G_2; t$
   and $\D$ is non-incremental
   \\
   and $G'$ is disjoint from $G_1$ and $G_2$
   \\
   then $\D' \derives \PreSt{G_1, G'}{p}{w} e !! G_2, G'; t$
   where $\D'$ is non-incremental.
\end{lem}
\begin{proof}
  By induction on $\D$.

  \begin{itemize}
      \ProofCasesRules{Eval-term, Eval-app, Eval-fix, Eval-bind,
                       Eval-case, Eval-split, Eval-fork, Eval-namespace, Eval-nest}

          These rules do not manipulate the graph, so
          just use the i.h.\ on each subderivation, then apply the same rule.

      \ProofCaseRule{Eval-refPlain}
           Since $\update{G_1}{q}{v}{G_2}$,
           we have $q \in \dom{G_2}$.
           \\ It is given that $\dom{G'} \disjoint \dom{G_2}$.
           Therefore $q \notin \dom{G_1, G'}$.
           \\ By definition, $\update{(G_1, G')}{q}{v}{(G_2, G')}$.
           \\ Apply Eval-refPlain.

      \ProofCaseRule{Eval-thunkPlain}
           Similar to the Eval-refPlain case.

      \ProofCaseRule{Eval-forcePlain}
         We have $G_1(q) = e_0$.  Therefore $(G_1, G')(q) = e_0$.
         Use the i.h.\ and apply Eval-forcePlain.

      \ProofCaseRule{Eval-getPlain}
         Similar to the Eval-forcePlain case.
  \qedhere
  \end{itemize}
\end{proof}



\subsection{Main result: From-scratch consistency}
\Label{sec:fsc}

At the highest level, the main result (\Theoremref{thm:fsc}) says:

\begin{quote}
\textbf{First approximation} \\
  If $\PreSt{H_1}{p}{w} e !! H_2; t$ by an incremental derivation,
  \\
  then $\PreSt{H_1'}{p}{w} e !! H_2'; t$,
  where $H_1'$ is a non-incremental version of $H_1$
  and $H_2'$ is a non-incremental version of $H_2$.
\end{quote}
%
Using the restriction function from \Sectionref{sec:restriction},
we can refine this statement:

\begin{quote}
\textbf{Second approximation} \\
  If  $\PreSt{H_1}{p}{w} e !! H_2; t$ by an incremental derivation
  and $P_1 \subseteq \dom{H_1}$,
  \\
  then $\PreSt{\restrict{H_1}{P_1}}{p}{w} e !! \restrict{H_2}{P_2}; t$
  by a non-incremental derivation,
  for some $P_2$ such that  $P_1 \subseteq P_2$.
\end{quote}
%
Here, the pointer set $P_1$ gives the scope of the non-incremental
input graph $\restrict{H_1}{P_1}$, and we construct $P_2$
describing the non-incremental output graph
$\restrict{H_2}{P_2}$.

We further refine this statement by involving the derivation's read- and
write-sets: the read set $R$ must be contained in $P_1$, the write set $W$
must be disjoint from $P_1$ (written $\dom{W} \disjoint P_1$), and $P_2$ must be
exactly $P_1$ plus $W$.
In the non-incremental semantics, the store should grow monotonically, so
we will also show $\restrict{H_1}{P_1} \subseteq \restrict{H_2}{P_2}$:

\begin{quote}
\textbf{Third approximation} \\
  If  $\PreSt{H_1}{p}{w} e !! H_2; t$ by an incremental derivation $\D$
  with $\DHasEffects{\D}{R}{W}$,
  \\
  and $P_1 \subseteq \dom{H_1}$
  such that $\dom{R} \subseteq P_1$
  and $\dom{W} \disjoint P_1$
  \\
  then $\PreSt{\restrict{H_1}{P_1}}{p}{w} e !! \restrict{H_2}{P_2}; t$
  \\
  where $\restrict{H_1}{P_1} \subseteq \restrict{H_2}{P_2}$
  and $P_2 = P_1 \cup \dom{W}$.
\end{quote}
%
Even this refinement is not quite enough, because the incremental
system can perform computations in a different order than the non-incremental
system.  Specifically, the Eval-computeDep rule carries out a subcomputation
first, then continues with a larger computation that depends on the subcomputation.
The subcomputation does not fit into the non-incremental derivation at that point;
non-incrementally, the subcomputation is performed when it is demanded by
the larger computation.  Thus, we can't just apply the induction hypothesis on the
subcomputation.

However, the subcomputation is ``saved'' in its (incremental) output graph.
So we incorporate an invariant that all thunks with cached results in the graph
``are consistent'', that is, they satisfy a property similar to the overall consistency
result.  When this is the case, we say that the graph is from-scratch consistent.
The main result, then, will assume that the input graph is from-scratch consistent,
and show that the output graph remains from-scratch consistent.
Since the graph can grow in the interval between the subcomputation of Eval-computeDep
and the point where the subcomputation is demanded, we require that the output
graph $G_2$ of the saved derivation does not contradict the larger, newer graph
$H$.  This is part (4) in the next definition.  (We number the parts from (i) to (ii)
and then from (1) so that they mostly match similar parts in the main result.)

\begin{defn}[From-scratch consistency of a derivation]
\Label{def:fsc}
~\\
  A derivation $\D_i \derives \PreSt{G_1}{p}{w} e !! G_2 ; t$
  is
  \\
  \emph{from-scratch consistent for}
  $P_q \subseteq \dom{G_1}$
  \emph{up to}
  $H$  % ``future'' context
  if and only if
  %
  \begin{enumerate}[(i)]
%  \item % i
%       $[[G1 wf]]$
  \item % ii
       $\D_i \satisfactory$ where $\DHasEffects{\D_i}{R}{W}$
  \item % iii
%     for all $[[P1]]$ such that
     $\dom{R} \subseteq P_q$
     and
     $\dom{W} \disjoint P_q$

      \item[(1)] % 1
           there exists a non-incremental derivation
           $\D_{ni}
            \derives
            \PreSt{\restrict{G_1}{P_q}}{p}{w} e !! \restrict{G_2}{P_2} ; t $

      \item[(2)] % 2
           $\restrict{G_1}{P_q} \subseteq \restrict{G_2}{P_2}$

      \item[(3)] % 3
           $P_2 = P_q \cup \dom{W}$

      \item[(4)] % 4
            $\restrict{G_2}{P_2} \subseteq \restrict{H}{\dom{H}}$
  \end{enumerate}
\end{defn}


\begin{defn}[From-scratch consistency of graphs]
\Label{def:fsc-graph}
~\\
A graph $H$ is
\emph{from-scratch consistent}
\\
if, for all $q \in \dom{H}$ such that $H(q) = (e,t)$,
     \\
     there exists
     $\D_q \derives \PreSt{G_1}{p}{w} e !! G_2 ; t$
     \\
     and
     $P_q \subseteq \dom{G_1}$
     \\
     such that $\D_q$ is from-scratch consistent (\Definitionref{def:fsc})
     for $P_q$ up to $H$.
\end{defn}


The proof of the main result must maintain that the graph is from-scratch
consistent as the graph becomes larger, for which \Lemmaref{lem:fsc-ext-graph}
is useful.

\begin{lem}[Consistent extension]
\Label{lem:fsc-ext}
~\\
  If  $\D_q$ is from-scratch consistent for $P_q$ up to $H$
  \\
  and $H \subseteq H'$
  \\
  then $\D_q$ is from-scratch consistent for $P_q$ up to $H'$.
\end{lem}
\begin{proof}
  Only part (4) of \Definitionref{def:fsc} involves the ``up to'' part
  of from-scratch consistency,
  so we already have (i)--(iii) and (1)--(3).

  We have (4) $\restrict{G_2}{P_2} \subseteq \restrict{H}{\dom{H}}$.
  Using our assumptions, $\restrict{H}{\dom{H}} \subseteq \restrict{H'}{\dom{H'}}$.

  Therefore (4) $\restrict{G_2}{P_2} \subseteq \restrict{H'}{\dom{H'}}$.
\end{proof}


\begin{lem}[Consistent graph extension]
\Label{lem:fsc-ext-graph}
~\\
   If $H$ is from-scratch consistent
   \\
   and $H \subseteq H'$
   \\
   and, for all $q \in \dom{H'} - \dom{H}$ such that $H'(q) = (e,t)$,
   \\
   $~~$  there exists
     $\D_q \derives \PreSt{G_1}{p}{w} e !! G_2 ; t$
     and
     $P_q \subseteq \dom{G_1}$
     \\
     $~~$
     such that $\D_q$ is from-scratch consistent (\Definitionref{def:fsc})
     \\
     $~~$
     for $P_q$ up to $H'$,
   \\
   then
   $H'$ is from-scratch consistent.
\end{lem}
\begin{proof}
  Use \Lemmaref{lem:fsc-ext} on each ``old'' pointer with a cached result in $H$,
  then apply the definitions for each ``new'' pointer with a cached result in
  $\dom{H'} - \dom{H}$.
\end{proof}

At last, we can state and prove the main result, which corresponds to
the ``third approximation'' above, plus the invariant that the graph is
from-scratch consistent (parts (iii) and (4)).

We present most of the proof in a line-by-line style, with the judgment or
proposition being derived in the left column, and its justification in the right column.
In each case, we need to show four different things (1)--(4), some of which are obtained
midway through the case, so we highlight these with ``(1) \Hand'', and so on.

\begin{thm}[From-scratch consistency]
\Label{thm:fsc}
~\\
  Given an incremental $\D_i \derives \PreSt{H_1}{p}{w} e !! H_2 ; t $ where
  \begin{enumerate}[(i)]
%  \item % (i)
%       $[[H1 wf]]$
  \item % (i)
       $\D_i \satisfactory$ where $\DHasEffects{\D}{R}{W}$
  \item % (ii)
     a set of pointers $P_1 \subseteq \dom{H_1}$ is such that $\dom{R} \subseteq P_1$ and $\dom{W} \disjoint P_1$
  \item % (iii)
     $H_1$ is from-scratch consistent (\Definitionref{def:fsc-graph})
%     \\
%     and $[[(restrict Gq' Pq) subseteq (restrict H1 P1)]]$
  \end{enumerate}
  then
  \begin{enumerate}[(1)]
  \item % (1)
    there exists a non-incremental
      $\D_{ni} \derives \PreSt{\restrict{H_1}{P_1}}{p}{w} e !! \restrict{H_2}{P_2} ; t$
  \item % (2)
      $\restrict{H_1}{P_1} \subseteq \restrict{H_2}{P_2}$
  \item % (3)
       $P_2 = P_1 \union \dom{W}$
  \item % (4)
      $H_2$ is from-scratch consistent (\Definitionref{def:fsc-graph}).
  \end{enumerate}
\end{thm}


% Local Variables:
% mode: latex
% TeX-master: "typed-adapton"
% End:


==> meta.tex <==
\section{Metatheory of \calc}
\label{sec:metatheory}

Ideally, we can use well-typedness to discharge certain conditions on the earlier
from-scratch consistency result.  To review, those conditions were:

\begin{itemize}
\item Theorem B.13 precondition (i):

  The evaluation derivation is \emph{globally satisfactory} (Def.\ B.7):
  
  \begin{itemize}
  \item All subderivations are \emph{locally satisfactory} (Def.\ B.6):
    \begin{itemize}
    \item The input graph is well-formed.  Def.\ B.6 (1)
    \item The output graph is well-formed.  Def.\ B.6 (1)
    \item ``$\Dee$ reads $R$ writes $W$'' is defined.  Def.\ B.6 (2)
    \end{itemize}
  \end{itemize}

\item Theorem B.13 precondition (ii):

  Something that relates a set of pointers $P_1$ to $R$ and $W$.

\item Theorem B.13 precondition (iii):

  The input \emph{graph} $H$ is \emph{from-scratch consistent} (Def.\ B.10):

  \begin{itemize}
  \item For all $q \in H$ such that $H(q) = (e, t)$,
    there exists an evaluation derivation $\Dee_e$ of $e$ from $G_1$ to $G_2$ such that
    $\Dee_e$ is from-scratch consistent (B.9) for $P_q$ up to $H$.

    \begin{itemize}
    \item A \emph{derivation} is \emph{from-scratch consistent}
      if \dots

      \begin{itemize}
      \item The derivation is satisfactory (which implies that $R$ and $W$ are defined).  Def.\ B.9 (i)
      \item $P_q$ is properly related to $R$ and $W$.  Def.\ B.9 (ii)
      \item There is a non-incremental derivation\dots ~~Def.\ B.9 (1)
      \item \dots whose graphs are consistent with the incremental graphs.  Def.\ B.9 (2), (3), (4)
      \end{itemize}
    \end{itemize}
  \end{itemize}
\end{itemize}

\begin{conjecture}
~\\
  If
  [$\Gamma$ well-formed]
  \\
  and
  [input graph well-formed]
  \\
  and
  [typing judgment]
  \\
  and
  [evaluation judgment]
  \\
  then
  [globally satisfactory].
\end{conjecture}

Can we also show B.13 (ii) and (iii)?  Do we need to show them?


% Local Variables: 
% mode: latex
% TeX-master: "types"
% End: 



==> mk <==
#!/bin/sh

killall latex
\rm *.aux
latex typed-adapton
bibtex typed-adapton
latex typed-adapton


==> pull-abstract <==
#!/bin/sh

# Script to extract the contents of \begin{abstract}...\end{abstract},
# strip newlines (preserving paragraph breaks), remove multiple blank lines,
# remove \emph{} markup,
# remove leading spaces, and remove newlines at end of file.
#
# Usage:
#  pull-abstract
#
# Creates abstract.txt from abstract.tex
#
# sources: various, including http://sed.sourceforge.net/sed1line.txt

if [ "$(uname -s)" == "Darwin" ] # If the system is Mac OS X
then
  sed=gsed
else
  sed=sed
fi

cat abstract.tex \
  | $sed -e 's/^ *//' \
  | $sed -e 's/\\emph{\([^}]*\)}/\1/g' \
  | $sed -e 's/\\@//g' \
  | $sed -e 's/\$\\lambda\$/lambda/g' \
  | $sed -e 's/\$\\beta\$/beta/g' \
  | $sed -e 's/\$\\eta\$/eta/g' \
  | $sed -e 's/\\"{o}/oe/g' \
  | $sed -e 's/\\"o/oe/g' \
  | $sed -e 's/\\citet{siek15criteria}/Siek et al. (2015)/g' \
  | $sed -e 's/\$\\times\$/x/g' \
  | $sed -e 's/``/"/g' \
  | $sed -e "s/''/\"/g" \
  | $sed -e '1,/begin{abstract}/ d' \
  | $sed -e '/end{abstract}/,$ d' \
  | $sed -e '/^%.*$/ d' \
  | $sed -e 's/%.*$//' \
  | $sed -e 's/^ *$/\$/' \
  | $sed -e ':a;N;$!ba;s/\n/ /g' \
  | $sed -e 's/\$/\n\n/g' \
  | $sed -e 's/^  *//' \
  | $sed -e :a -e '/^\n*$/{$d;N;ba' -e '}' \
  > abstract.txt


==> pull-abstract-html <==
#!/bin/sh

# Script to extract the contents of \begin{abstract}...\end{abstract},
# strip newlines (preserving paragraph breaks), remove multiple blank lines,
# HTMLify \emph{} markup,
# remove leading spaces, and remove newlines at end of file.
#
# Usage:
#  pull-abstract
#
# Creates abstract.html from abstract.tex
#
# sources: various, including http://sed.sourceforge.net/sed1line.txt

if [ "$(uname -s)" == "Darwin" ] # If the system is Mac OS X
then
  sed=gsed
else
  sed=sed
fi

cat abstract.tex \
  | $sed -e 's/^ *//' \
  | $sed -e 's/\\emph{\([^}]*\)}/<i>\1<\/i>/g' \
  | $sed -e 's/\\@//g' \
  | $sed -e 's/\$\\lambda\$/\&lambda;/g' \
  | $sed -e 's/\$\\times\$/\&times;/g' \
  | $sed -e 's/\\Adapton/Adapton/g' \
  | $sed -e 's/\\NominalAdapton/Nominal Adapton/g' \
  | $sed -e 's/\\citet{siek15criteria}/Siek et al. (2015)/g' \
  | $sed -e '1,/begin{abstract}/ d' \
  | $sed -e '/end{abstract}/,$ d' \
  | $sed -e 's/``/\&ldquo;/g' \
  | $sed -e "s/''/\&rdquo;/g" \
  | $sed -e 's/`/\&lsquo;/g' \
  | $sed -e "s/'/\&rsquo;/g" \
  | $sed -e '/^%.*$/ d' \
  | $sed -e 's/%.*$//' \
  | $sed -e 's/^ *$/\$/' \
  | $sed -e ':a;N;$!ba;s/\n/ /g' \
  | $sed -e 's/\$/\n<p>\n/g' \
  | $sed -e 's/^  *//' \
  | $sed -e :a -e '/^\n*$/{$d;N;ba' -e '}' \
  > abstract.html

